Improving Unsupervised Constituency Parsing via Maximizing Semantic Information

Unsupervised constituency parsers organize phrases within a sentence into a tree-shaped syntactic constituent structure that reflects the organization of sentence semantics. However, the traditional objective of maximizing sentence log-likelihood (LL) does not explicitly account for the close relationship between the constituent structure and the semantics, resulting in a weak correlation between LL values and parsing accuracy. In this paper, we introduce a novel objective that trains parsers by maximizing SemInfo, the semantic information encoded in constituent structures. We introduce a bag-of-substrings model to represent the semantics and estimate the SemInfo value using the probability-weighted information metric. We apply the SemInfo maximization objective to training Probabilistic Context-Free Grammar (PCFG) parsers and develop a Tree Conditional Random Field (TreeCRF)-based model to facilitate the training. Experiments show that SemInfo correlates more strongly with parsing accuracy than LL, establishing SemInfo as a better unsupervised parsing objective. As a result, our algorithm significantly improves parsing accuracy by an average of 7.85 sentence-F1 scores across five PCFG variants and in four languages, achieving state-of-the-art level results in three of the four languages.

==> src/contents/arxiv/method-v0.tex <==
----------------------------

\<just so hard to explain this part\>
\<!!string as a carrier of information\>
\<regularity observed in string generation is the information\>

Figure \ref{} illustrates our modeling of the sentence generation process.
In this process, the semantics is a latent variable whereas the sentence is an observed variable.
Given a semantics, we can sample multiple sentences that are superficially different but encode the same semantics.
This model captures the phenomenon that human can express the same idea in different ways through paraphrasing.
We refer to the sampled sentences as paraphrastic sentences\footnote{Because these sentences are generated as a result of paraphrasing.}.




\subsection{Bag-of-Maximal-Substring Model}
In this section, we define the probability $P(s|Sem(x))$ of a substring $s$ being generated to encode $x$'s semantic information $Sem(x)$.



\<strings generated to carry information\>
We hypothesize that semantic information are encoded in the string or substrings of sentences.
Given a sentence, humans can decode the semantics observing the whole string or a substring of the sentence.
However, such capability does not extend to arbitrary substrings.
For example, a sentence ``John has been working on a theory until 5 p.m. tonight'' and one of its substring ``has been working on a theory'' can be decoded. 
But substrings such as ``has been'' or ``working on'' can not.
This indicates 

Human is an interesting machine.
They can partially decode the semantics using a substring of a sentence.
However, they are incapable of decoding the semantics from arbitrary substrings.
This phenomenon indicates a potential gap in information that substrings encode about the semantics.


\subsection{Maximal Substrings: String Generated by semantic needs}
\<assume: substring as carrier of information\>
By Chomsky's sacred word, constituents are significant substrings in natural language sentences \cite{}.
We interpret the significance as the substring's ability to carry semantic information.
That means the substring needs to be repeatedly generated across the paraphrastic string set to preserve the semantic information.
We identify the significant substring as the maximal substring in two paraphrastic sentences $x_1$ and $x_2$.

\begin{equation}
    MS(x_1, x_2):=\{x: x\leq x_1\wedge x\leq x_2\wedge \forall x^\prime (x<x^\prime \implies \neg x^\prime \leq x_1 \vee \neg x^\prime \leq x_2) \}
\end{equation}

The motivation of introducing the maximal substring is to ensure that the generation of the substring is caused by the need to replicate the semantic information.
Let's consider two paraphrastic strings: ``John has been working on a theory until 5 p.m. tonight'' and ``John, until 5 p.m. tonight, has been working on a theory''. 
A maximal substring is ``has been working on a theory'', encoding the semantic information that someone is working on a theory.
However, similar semantic information might be absent in non-maximal substrings, such as ``has been'' or ``on a''.
This is because the non-maximal substring is generated as a consequence of the maximal substring being generated.
We can make similar observation to another maximal substring ``until 5 p.m. tonight''.
Excluding the non-maximal substring can exclude observations of string generations casued by non-semantic factors.














\subsection{Maximal String as Observation to $Sem(x)$}
In this paper, we employ maximal strings as a proxy to observe the sentence semantics.




Despite being an fundamental element of natural language, sentence semantics are not observable, posing a significant challenge in measuring the SemInfo value.
In this paper, we observe the semantics through a set of paraphrastic sentence strings.







In this paper, we observe the semantics through a set of periphrastic sentence strings.






\begin{wrapfigure}{r}{0.3\textwidth} %this figure will be at the right
    \centering
    \includegraphics[width=0.3\textwidth]{src/figures/ICLR25-langgen.drawio.pdf}
    \caption{Sentence Generation Process}
\end{wrapfigure}





\<observe the semantics through the repeated sampled sentences\>


In natural languege communications, one can convey the same thought with vastly different sentences strings.
The variation in the sentence string may manifest as changes in word usages or changes in word order. 
Despite the superficial variation, those sentence strings still encodes the same semantic information.
This means 




may include changes in word usage, changes in word order, or even  
Despite the difference in the sentence string, 

We formalize the 






\<communication\>
Natural language is a tool of communication.
Natural language sentences serve as a carrier of semantic information that we, as the sender of information, want to deliver.
\<paraphrases\>




% We estimate $\log\frac{P(Sem(x)|s)}{P(Sem(x)}$ with $\log \frac{|s\leq x^\prime :x^\prime\sim \mathcal{D}|}{|\mathcal{D}|}$, the inverse sentence frequency of $\gD$ generating $s$ as a substring.
% We use $\alpha\leq\beta$ to denote the partial order relationship of $\alpha$ being a substring of $\beta$ and $\alpha\leq\beta$ to denote $\alpha$ being a proper substring of $\beta$.

\begin{align}
    tfidf(s, Sem(x)) &= P(Sem(x))P(s|Sem(x))\log \frac{P(Sem(x)|s)}{P(Sem(x))}\\
    \intertext{where}
    P(Sem(x)) = \frac{1}{|\gD|}
\end{align}

% <bag-of-string model>
% % Now that the problem is to find out substrings with high semantic information, the task is to develop a metric. 
% The key problem here is to measure the information between substrings and semantics.
% We apply the informtion-theoretic metrics (background) developed for bag-of-word models for this purpose.
% <term information is proportional to term frequency> <- BoW
% We develop a bag-of-string model....
% Intuitively, a substring with higher frequency would indicate a higher semantic information.
% \<what is a bag-of-string\>
% The need to define $P(s|Sem)$


% Driven by the need to replicate the semantics, a substring carrying high semantic information is more likely to be \textit{regenerated as a substring} of paraphrases in a paraphrasing process depicted in Fig~\ref{}.
% In this process, we denote the source sentence to the paraphrasing process by $x$ and substrings to $x$ by $s$.
% For each $x$, we gain access to its semantics $Sem()$ as a latent variable.
% We can sample paraphrases $(x_1, x_2,...)$ from $Sem(x)$ but cannot directly observe $Sem(x)$.
% We denote the set of paraphrases by  $\{x_i\}$.
% The paraphrasing process provides a means to measure the string-semantics information by modeling $P(s|Sem(x))$, the probability of $s$ being generated as a substring to replicate the semantics $x$.

==> src/tbl/correlation-tbl.tex <==
\begin{wraptable}{r}{0.5\textwidth}
    \centering
    \begin{adjustbox}{width=0.5\textwidth}
    \begin{tabular}{l|c|c|c}
    \hline
         & SemInfo-\isfo & LL-\isfo & SemInfo-LL \\ \hline
        CPCFG & 0.6518 & 0.0223 & 0.0196 \\ 
        NPCFG & 0.6347 & -0.0074 & -0.0045 \\ 
        SCPCFG & 0.6431 & -0.0013 & 0.0505 \\ 
        SNPCFG & 0.9289 & 0.0102 & 0.0182 \\ 
        TNPCFG & 0.6449 & 0.1077 & 0.1426 \\ \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Spearman correlation coefficient between SemInfo, \isfo, and LL over the English validation set. Correlations are computed on a sentence-level and aggregated in the corpus-level.}
\end{wraptable}


==> src/tbl/instance-level-ttest.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|ccccc}
    \hline
        ~&NPCFG & SNPCFG & TNPCFG & CPCFG & SCPCFG \\ \hline
        English & 42.74 & 27.62 & 39.78 & 37.06 & 56.91 \\ 
        Chinese & 43.41 & 30.98 & 26.04 & -4.12 & 21.83 \\ 
        German & 21.03 & 39.09 & 18.86 & 17.95 & 11.11 \\ 
        French & 12.74 & 15.8 & 39.31 & 13.26 & 22.24 \\ \hline
    \end{tabular}
    \caption{T-statistics of t-tests evaluating if SemInfo-trained PCFG parsers' \isfo 
 is different from LL-trained PCFG parsers' \isfo. A positive t-statistics indicates that the SemInfo-trained PCFG significantly outperforms the LL-trained PCFG. A negative t-statistics indicates the SemInfo-trained PCFG significantly outperforms the LL-trained PCFG.}
    \label{tbl:ttest-instance_level}
\end{table}

==> src/tbl/validation-tbl.tex <==
\begin{table}[t]
    % \tiny
    \centering
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{cc|cc|cc|cc|cc}
    \hline
        & & English & $\Delta$ & Chinese & $\Delta$ & French & $\Delta$ & German & $\Delta$ \\ \hline
        \multirow{2}{*}{CPCFG}&SemInfo & 65.74±0.03 & \multirow{2}{*}{8.06} & 51.62±0.38 & \multirow{2}{*}{0.77} & 52.51±0.46 & \multirow{2}{*}{6.19} & 49.35±0.42 & \multirow{2}{*}{4.25} \\ %\cline{2-10}
        &LL & 57.68±1.15 &  & 50.85±2.71 &  & 46.32±0.61 &  & 45.09±1.10 &  \\ \hline
        \multirow{2}{*}{NPCFG}&SemInfo & 66.96±0.57 & \multirow{2}{*}{13.05} & 53.67±0.71 & \multirow{2}{*}{11.96} & 52.69±0.78 & \multirow{2}{*}{5.27} & 50.57±0.55 & \multirow{2}{*}{4.05} \\ %\cline{2-10}
        &LL & 53.90±2.97 &  & 41.71±2.73 &  & 47.42±0.61 &  & 46.52±1.31 &  \\ \hline
        \multirow{2}{*}{SCPCFG}&SemInfo & 66.25±0.39 & \multirow{2}{*}{20.28} & 51.28±0.56 & \multirow{2}{*}{4.11} & 54.18±0.68 & \multirow{2}{*}{11.18} & 48.34±1.13 & \multirow{2}{*}{2.41} \\ %\cline{2-10}
        &LL & 45.97±2.62 &  & 47.18±0.45 &  & 43.00±1.69 &  & 45.93±1.21 &  \\ \hline
        \multirow{2}{*}{SNPCFG}&SemInfo & 67.01±0.57 & \multirow{2}{*}{11.67} & 51.52±0.45 & \multirow{2}{*}{6.44} & 55.12±0.83 & \multirow{2}{*}{6.71} & 49.52±0.73 & \multirow{2}{*}{8.51} \\ %\cline{2-10}
        &LL & 55.34±3.38 &  & 45.09±1.12 &  & 48.41±0.78 &  & 41.01±0.95 &  \\ \hline
        \multirow{2}{*}{TNPCFG}&SemInfo & 65.25±0.53 & \multirow{2}{*}{12.20} & 50.50±1.02 & \multirow{2}{*}{9.22} & 54.58±1.43 & \multirow{2}{*}{9.45} & 50.53±0.28 & \multirow{2}{*}{2.14} \\ %\cline{2-10}
        &LL & 53.05±1.14 &  & 41.29±4.52 &  & 45.13±1.72 &  & 48.39±0.20 &  \\ \hline\hline
        % &~ & ~ & 13.05 & ~ & 6.50 & ~ & 7.76 & ~ & 4.27 \\ \hline
        % &~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        \multicolumn{2}{c|}{Spanoverlap} & 57.42 & ~ & 49.22 & ~ & 50.64 & ~ & 49.4 & ~ \\ \hline
        \multicolumn{2}{c|}{GPT4o-mini} & 36.16 & ~ & 11.82 & ~ & 30.01 & ~ & 33.56 & ~ \\ \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Sentence-F1 score of five PCFG variants trained with the SemInfo Maximization objective and the LL Maximization objective. THis }
\end{table}
